Sample-Efficient Robust Multi-Agent Reinforcement Learning in the Face of Environmental Uncertainty

To overcome the sim-to-real gap in reinforcement learning (RL), learned policies must maintain robustness against environmental uncertainties. While robust RL has been widely studied in single-agent regimes, in multi-agent environments, the problem remains understudied -- despite the fact that the problems posed by environmental uncertainties are often exacerbated by strategic interactions. This work focuses on learning in distributionally robust Markov games (RMGs), a robust variant of standard Markov games, wherein each agent aims to learn a policy that maximizes its own worst-case performance when the deployed environment deviates within its own prescribed uncertainty set. This results in a set of robust equilibrium strategies for all agents that align with classic notions of game-theoretic equilibria. Assuming a non-adaptive sampling mechanism from a generative model, we propose a sample-efficient model-based algorithm (DRNVI) with finite-sample complexity guarantees for learning robust variants of various notions of game-theoretic equilibria. We also establish an information-theoretic lower bound for solving RMGs, which confirms the near-optimal sample complexity of DRNVI with respect to problem-dependent factors such as the size of the state space, the target accuracy, and the horizon length.

==> extension.tex <==
%!TEX root = ./RobustMARL-icml.tex

\section{Open problem/possible extensions}




\subsection{Extension to $s$-rectangularity finite-sample bound}
In this work, we may focus on $(s,a)$-rectangularity, which is a simpler case than $s$-rectangularity. So it is very interesting to study how to solve the game in $s$-rectangularity cases. In such cases, we have an additional set of $m$ natural adversarial players that try to minimize each agent's performance conditioned on all agents' policy.




\subsection{Extension to robust offline MARL}
It seems for offline setting, we can break the curse of dimension just like \citet{li2023minimax}. Can make this as journal extension.


\subsection{Extension to reward-agnostic robust MARL}
It seems for offline setting, we can break the curse of dimension just like \citet{li2023minimax}. Can make this as journal extension.


\subsection{A tighter lower bound for Nash equilibrium}
For lower bound, is there any work that shows the sample complexity lower bound for computing CCE? only found some for computing Nash \citep{zhang2020model,song2021can}.




\subsection{Upper bound for Robust Markov games with $(s, a_i, \pi(s))$-rectangularity}


\subsection{Upper bound for Robust Markov games with $(s, \pi(s))$-rectangularity}
\lxs{No existence of Nash equilibrium. And no CCE/CE (at least now can't find some proof for that)}

To begin with, we introduce some additional notations. For any transition kernel $P =\{P_h\}_{1\leq h\leq H}$ (resp.~ the nominal transition kernel $P^\no$), any policy $\pi$, we have for any agent, they have a same uncertainty set defined as below:
\begin{align}
&P^{\pi}_{h,s}(s') = \mathbb{E}_{\ba\in \pi_{h}(s)} \left[ P_h(s'\mymid s, \ba)\right] \quad \text{and} \quad P^{\no,\pi}_{h,s}(s') = \mathbb{E}_{\ba\in \pi_h(s)} \left[ P^{\no}_h(s'\mymid s, \ba)\right].
\end{align}
For a fixed policy $\pi_{-i}$, we represent the above quantity w.r.t. the policy of the i-th player $\pi_i$ as 
\begin{align}
&P^{\pi_i \times \pi_{-i}}_{h,s}(s') =\mathbb{E}_{a_i\in\pi_{i,h}(s)} \mathbb{E}_{\ba_{-i}\in \pi_{-i,h}(s)} \left[ P_h(s'\mymid s, a_i, \ba_{-i})\right] = \mathbb{E}_{a_i\in\pi_{i,h}(s)} \left[P^{\pi_{-i}}_h(s,a_i)\right], \\
&P^{\no,\pi_i \times \pi_{-i}}_{h,s}(s') = \mathbb{E}_{a_i\in\pi_{i,h}(s)} \mathbb{E}_{\ba_{-i}\in \pi_{-i,h}(s)} \left[ P^{\no}_h(s'\mymid s, a_i, \ba_{-i})\right] = \mathbb{E}_{a_i\in\pi_{i,h}(s)} \left[P^{0, \pi_{-i}}_h(s, a_i)\right],
\end{align}
where
\begin{align}
\quad P^{\pi_{-i}}_h(s,a_i) = \mathbb{E}_{\ba_{-i}\in \pi_{-i,h}(s)} \left[ P_h(s'\mymid s, a_i, \ba_{-i})\right] \quad \text{and} \quad P^{0, \pi_{-i}}_h(s, a_i) = \mathbb{E}_{\ba_{-i}\in \pi_{-i,h}(s)} \left[ P^{\no}_h(s'\mymid s, a_i, \ba_{-i})\right]. 
\end{align}

Then we introduce the uncertainty set.
In particular, given the nominal transition kernel $P^\no$, any joint policy $\pi = \{\pi_{i,h}\}_{1\leq i\leq n, h\in[H]}$, and some uncertainty level $\ror$, the uncertainty set---with $\ell_p(\cdot)$ as the divergence metric $\rho: \Delta(\cS) \times \Delta(\cS) \rightarrow \mathbb{R}^+$---is specified as
\begin{align}\label{eq:general-infinite-P}
	\cU_\rho^{\ror}(P^{\no},\pi) &\defn \otimes \; \cU_\rho^{\ror}(P^{\no,\pi}_{h,s})\qquad \text{with}\quad
	\cU_\rho^{\ror}(P^{\no,\pi}_{h,s}) \defn \left\{ P_{h,s} \in \Delta (\cS):  \left\|P_{h,s}- P^{\no,\pi}_{h,s}\right\|_p \leq \ror \right\}.
\end{align}
\begin{remark}
1) Here, each $P_{h,s}$ that belongs to the uncertainty set actually represent the overall effect of the perturbed transition kernel $P_{h,s,\ba}$ for all $(s,\ba)$ without explicitly say how to change each one of them.

2) Note that now the uncertainty set at each state $s$ is not fixed (determined by $\rho$ and $\sigma$), but also \textcolor{red}{depends on the joint policy $\pi$} of all agents.
\end{remark}

Now we can define the corresponding value function/ Q-function as
\begin{align}
V_{i,h}^{\pi}(s) &\defn  \inf_{P\in \cU_\rho^{\ror}(P^{\no},\pi)} \mathbb{E}_{P,\pi}\left[\sum_{t=h}^{T} r_{i,t}(s_t, \ba_t) \mymid s_h = s\right],\\
 \quad Q_{i,h}^{\pi}(s, \ba) &\defn  \inf_{P\in \cU_\rho^{\ror}(P^{\no},\pi)} \mathbb{E}_{P,\pi}\left[\sum_{t=h}^{T} r_{i,t}(s_t, a_t) \mymid s_h =s, \ba_h = \ba \right].
\end{align}

Therefore, we have the Bellman consistency equation and Bellman optimality equation (to be checked)
\begin{align}
V_{i,h}^{\pi}(s) = \mathbb{E}_{\ba\in \pi(s)}\left[ r_{i,h}(s,\ba)\right] + \inf_{P\in \cU_\rho^{\ror}(P^{\no,\pi}_{h,s})} P V_{i,h+1}^{\pi}, \\
Q_{i,h}^{\pi}(s, \ba) = r_{i,h}(s,\ba) + \text{argmin}_{P\in \cU_\rho^{\ror}(P^{\no,\pi}_{h,s})} P_{h,s,\ba} V_{i,h+1}^{\pi}. \label{payoff}
\end{align}



Fixing the other agents' policy $\pi_{-i}$, we can define the {\em robust best-response} value function as following:
\begin{align}
V_{i,h}^{\star, \pi_{-i}}(s) &= \max_{\pi_{i,h} \in \Delta(\cA_i)}  \inf_{ P \in \cU^\ror(P^\no, \pi_i \times \pi_{-i})} \Big\{ \mathbb{E}_{a_i \times \ba_{-i} \sim \pi_{i,h} \times \pi_{-i,h}}\left[ r_{i,h}(s,\ba) +  P_{h,s,\ba} V_{i,h+1}^{\star, \pi_{-i}} \right]\Big\} \\
& = \max_{\pi_{i,h} \in \Delta(\cA_i)}  \Big\{ \mathbb{E}_{a_i \times \ba_{-i} \sim \pi_{i,h}(s) \times \pi_{-i,h}(s)}\left[ r_{i,h}(s,\ba)\right] + \inf_{P\in \cU_\rho^{\ror}(P^{\no,\pi_i\times \pi_{-i}}_{h,s})} P V_{i,h+1}^{\star, \pi_{-i}} \Big\} \\
& = \max_{\pi_{i,h} \in \Delta(\cA_i)}  \Big\{ \mathbb{E}_{a_i\sim \pi_{i,h}} [\mathbb{E}_{\ba_{-i}  \sim \pi_{-i,h}}\left[ r_{i,h}(s, a_i, \ba_{-i})\right]] + \inf_{P\in \cU_\rho^{\ror}(\mathbb{E}_{a_i\in\pi_{i,h}(s)} \left[P^{0, \pi_{-i}}_h(s, a_i)\right])} P V_{i,h+1}^{\star, \pi_{-i}} \Big\} \\
& = \max_{\pi_{i,h} \in \Delta(\cA_i)}  \Big\{ \mathbb{E}_{a_i\sim \pi_{i,h}} \left[r^{\pi_{-i}}_{i,h}(s, a_i)\right] + \inf_{P\in \cU_\rho^{\ror}(\mathbb{E}_{a_i\in\pi_{i,h}(s)} \left[P^{0, \pi_{-i}}_h(s, a_i)\right])} P V_{i,h+1}^{\star, \pi_{-i}} \Big\} 
\end{align}



\subsubsection{About Nash equilibrium.}

\paragraph{I: Finite-game has Nash.}
Using the following theorem, we have the existence of Nash equilibrium:
\begin{theorem}[Nash'51]
 Every game with finite set of players and finite pure strategy sets has at least
one (mixed) Nash Equilibrium.
\end{theorem}

But the problem is that we are not a finite-game, since each agent has infinite pure strategy within a simplex, i.e., the $i$-th player can choose a mixed strategy over $\Delta(\cA_i)$ (a finite-dimensional simplex). The payoff function is also defined for joint mixed strategy $\pi \in \Delta(\cA)$, but no longer a joint pure strategy:
\begin{align}
V_{i,h}^{\pi}(s) = \mathbb{E}_{\ba\in \pi(s)}\left[ r_{i,h}(s,\ba)\right] + \inf_{P\in \cU_\rho^{\ror}(P^{\no,\pi}_{h,s})} P V_{i,h+1}^{\pi} = \mathbb{E}_{\ba\sim \pi(s)}[Q_{i,h}^{\pi}(s, \ba)] \neq \mathbb{E}_{\ba\sim \pi(s)}[Q_{i,h}^{\ba}(s, \ba)].
\end{align}



\paragraph{II: Continuous game has a mixed Nash equilibrium}
\begin{theorem}[Nash'51]
 Every continuous game with finite set of players and infinite pure strategy sets has at least
one (mixed) Nash Equilibrium.
\end{theorem}

The problem is that a mixed Nash equilibrium for us is a distribution over the simplex $\Delta(\cA_i)$, which means nothing.

But Kakutani's fixed-point theorem can ensure a pure strategy Nash equilibrium, which is what we want.


\paragraph{III: Kakutani's fixed point theorem won't work: loss the convexity of $\phi(x)$.}
Now the answer for Nash is no. Since by Kakutani's fixed point theorem, we need to ensure
\begin{itemize}
	\item X is closed, bounded, and convex set in Euclidean space. 
	{\em Satisfied since $x = \pi$, i.e., the joint policy of all agents, and $X = \Delta(\cA_1) \times \Delta(\cA_2) \times \cdots \times \Delta(\cA_n)$ is a product of simplexes. }
	\item the mapping $\phi(x)$ is an upper semicontinuous corresponding mapping.
	{\em Here, $x=\pi$, 
	\begin{equation}
	\phi(\pi) = \{ \pi^\star \mymid \pi^\star_{i,h}(s) \in \arg\max_{\pi_i'} V_{i,h}^{\pi_i' \times \pi_{-i}}(s)\}_{1\leq i\leq n, 1\leq h\leq H, s\in \cS} 
	\end{equation}}
	We may have $\phi(\pi)$ is continuous w.r.t. $\pi$ for all $i,h,s$.

	\item $\phi(x)$ is a convex set.
	\textcolor{red}{This one can't be shown.} In particular, suppose that for time step $h$, there exists two Nash equilibrium $z = (z_1, \cdots, z_n), v = (v_1, \cdots, v_n) \in \phi(\pi)$.  Then we have that for any i-the player's policy $u_i \in \Delta(\cA_i)$,
	\begin{align}
	V_{i,h}^{\star, \pi_{-i}} = \max_{\pi_i'} V_{i,h}^{\pi_i' \times \pi_{-i}}(s) = V_{i,h}^{z_i \times \pi_{-i}}(s) =  V_{i,h}^{v_i \times \pi_{-i}}(s) \geq V_{i,h}^{u_i \times \pi_{-i}}(s).
	\end{align}

	Then we need to show that for any $\lambda\in [0,1]$, $\lambda z + (1-\lambda) v$ also $\in \phi(x)$, i.e.,
	\begin{align}
	V_{i,h}^{(\lambda z_i + (1-\lambda) v_i) \times \pi_{-i}}(s) = V_{i,h}^{\star, \pi_{-i}}(s).
	\end{align}
Towards this, we have
\begin{align}
V_{i,h}^{\star, \pi_{-i}}(s) &= \lambda  V_{i,h}^{z_i \times \pi_{-i}}(s) + (1-\lambda) V_{i,h}^{v_i \times \pi_{-i}}(s) \\
& = \lambda\left(\mathbb{E}_{a_i\sim z_{i,h}} \left[r^{\pi_{-i}}_{i,h}(s, a_i)\right] + \inf_{P\in \cU_\rho^{\ror}(\mathbb{E}_{a_i\in z_{i,h}(s)} \left[P^{0, \pi_{-i}}_h(s, a_i)\right])} P V_{i,h+1}^{\star, \pi_{-i}} \right) \\
&\quad + (1-\lambda)\left(\mathbb{E}_{a_i\sim v_{i,h}} \left[r^{\pi_{-i}}_{i,h}(s, a_i)\right] + \inf_{P\in \cU_\rho^{\ror}(\mathbb{E}_{a_i\in v_{i,h}(s)} \left[P^{0, \pi_{-i}}_h(s, a_i)\right])} P V_{i,h+1}^{\star, \pi_{-i}} \right)  \\
&= \mathbb{E}_{a_i\sim [\lambda z_{i,h} + (1-\lambda) v_{i,h}] } \left[r^{\pi_{-i}}_{i,h}(s, a_i)\right] + \lambda  \inf_{P\in \cU_\rho^{\ror}(\mathbb{E}_{a_i\in z_{i,h}(s)} \left[P^{0, \pi_{-i}}_h(s, a_i)\right])} P V_{i,h+1}^{\star, \pi_{-i}} \\
&\quad + (1-\lambda)  \inf_{P\in \cU_\rho^{\ror}(\mathbb{E}_{a_i\in v_{i,h}(s)} \left[P^{0, \pi_{-i}}_h(s, a_i)\right])} P V_{i,h+1}^{\star, \pi_{-i}}.
\end{align}

With the above expression, now we can compare to $V_{i,h}^{\star, \pi_{-i}}(s)$ to $V_{i,h}^{(\lambda z_i + (1-\lambda) v_i)}$, namely,
\begin{align}
&V_{i,h}^{\star, \pi_{-i}}(s) - V_{i,h}^{(\lambda z_i + (1-\lambda) v_i)} = \mathbb{E}_{a_i\sim [\lambda z_{i,h} + (1-\lambda) v_{i,h}] } \left[r^{\pi_{-i}}_{i,h}(s, a_i)\right] + \\
&\quad + \lambda \max_{\alpha \in [-H,H]}  \left[ \mathbb{E}_{a_i\in z_{i,h}(s)} \left[P^{0, \pi_{-i}}_h(s, a_i)\right] [V]_\alpha - \sigma(\alpha - \min{s'} [V]_\alpha (s'))\right]  \\
&\quad + (1-\lambda) \max_{\alpha \in [-H,H]}  \left[ \mathbb{E}_{a_i\in v_{i,h}(s)} \left[P^{0, \pi_{-i}}_h(s, a_i)\right] [V]_\alpha - \sigma(\alpha - \min{s'} [V]_\alpha (s'))\right] \\
&\quad -  \Big\{\mathbb{E}_{a_i\sim [\lambda z_{i,h} + (1-\lambda) v_{i,h}] } \left[r^{\pi_{-i}}_{i,h}(s, a_i)\right] \\
&\qquad + \max_{\alpha \in [-H,H]}  \left[ \mathbb{E}_{a_i\in \lambda z_{i,h}(s) + (1-\lambda) v_{i,h}(s)} \left[P^{0, \pi_{-i}}_h(s, a_i)\right] [V]_\alpha - \sigma(\alpha - \min{s'} [V]_\alpha (s'))\right]\Big\} \\
& \geq 0.
\end{align}

It shows that $\lambda z + (1-\lambda) v$ does not get the maximum robust value function, i.e., not belong to $\phi(\pi)$. Indeed, if we want to show $V_{i,h}^{\star, \pi_{-i}}(s) = V_{i,h}^{(\lambda z_i + (1-\lambda) v_i)}$, we need the inner problem $\inf(\cdot)$ be totally linear to the nominal transition kernel, which is not possible actually.
\lxs{The message shows that owing to the policy-dependent uncertainty set, we can't arrive at the convex of Nash equilibrium set. When we have a fixed uncertainty set, the opposite direction can be done, so we have $V_{i,h}^{\star, \pi_{-i}}(s) - V_{i,h}^{(\lambda z_i + (1-\lambda) v_i)} \leq 0$ so that $V_{i,h}^{\star, \pi_{-i}}(s) = V_{i,h}^{(\lambda z_i + (1-\lambda) v_i)}$. Then we have convexity of $\phi(\pi)$.}
\end{itemize}


\subsubsection{about CE/CCE.} The intuition that why CE/CCE may exists is that CCE/CE are convex set by the definition, which bypass the difficulty of showing the convexity of $\phi(\pi)$. So we may have some other way to prove the existence of CCE/CE.

The following theorem that shows the existence of both CE and CCE from this paper \citep{hart1989existence} which does not require the fixed point theorem seems solves our problem: 
\begin{theorem}
For each $i\in n$, the policy space $S^i$ is compact Hausdorff and the payoff function $h^i$ is continuous (where the joint policy space $S = \Pi_{1\leq i\leq n} S^i$ is endowed with the product topology). Let $\Sigma^i$ be the Borel $\sigma$-algebra on $S^i$, and let $\Sigma$ be the Borel $\sigma$-algebra on $S$. Then there exists a countably additive  correlated equilibrium with respect to $\{\Sigma^i\}_{1\leq i\leq n}$ and $\Sigma$.
\end{theorem}
	

So we have the existence of countably additive CE/CCE (\textcolor{red}{which actually is not enough}) since for each time step $h$, fixing the optimal value function $V_{i,h+1}^\star$, the one-step game satisfies (\textcolor{red}{need to be checked})
\begin{itemize}
	\item $S^i = \Delta(\cA_i)$ is a simplex, s.t. is compact and Hausdorff.
	\item the payoff function $h^i(\pi_h) = V_{i,h}^{\pi_h}$ is continuous:
	\begin{lemma}[$h^i$ is continuous]
	$\forall \epsilon>0$, there exists $\delta(\epsilon)>0$, s.t for any two joint policy $\pi^1(s), \pi^2(s)$, when $\max_{\ba\in \cA, 1\leq i\leq n} |\pi^1_{i,h}(s) - \pi^2_{i,h}(s)| = d(\pi^1(s), \pi^2(s)) \leq \delta(\epsilon)$, then 
	\begin{equation}
	 \left| V_{i,h}^{\pi^1_h}(s) - V_{i,h}^{\pi^2_h}(s)\right| \leq \epsilon.
	\end{equation}
	\end{lemma}

\begin{proof}
Recall the definition of the payoff function
\begin{align}
V_{i,h}^{\pi^1, V^{\star}_{i,h+1}}(s) &= \mathbb{E}_{\ba\in \pi^1_h(s)}\left[ r_{i,h}(s,\ba)\right] + \inf_{P\in \cU_\rho^{\ror}(P^{\no,\pi^1}_{h,s})} P V^{\star}_{i,h+1}.
\end{align}
The continuity is due to 1) the first term is linear to $\pi^1_h$ and 2) the uncertainty set in the second term depends on a nominal transition kernel $P^{\no,\pi^1}_{h,s} = \mathbb{E}_{\ba\in \pi^1_h(s)} \left[ P^{\no}_h(s'\mymid s, \ba)\right]$, which is also linear to $\pi^1_h$. 

\end{proof}

	\end{itemize}
